From array algebra to energy efficiency on GPUs: Data and hardware shapes with dimension-lifting to optimize memory-processor layouts

We present a new formulation for parallel matrix multiplication (MM) to out-perform the standard row-column code design. This algorithm is formulated in the MoA formalism (A Mathematics of Arrays) and combines an array view of hardware (dimension-lifting) to extend indexing to physical memory/processing units, with a contiguous data layout derived from static transformations. This view of a hardware-software model is thus a bridging model in the sense of Valiant's BSP. OpenACCcode was derived from the MoA expressions's normal form, producing optimal block sizes using the static information of types and shapes. Experiments were run on Nvidia V100 GPUs and reveal energy consumption which is quadratic in N, i.e. linear in the size of matrix. More generally this approach may be an ideal way of formulating, optimizing, and mapping array algorithms to embedded hardware. This work builds upon recently published results of NREL scientists. .

==> moa_basic.tex <==
\subsection{Appendix: MoA, functional combinators for arrays}

\footnote{The reader preferring an overview is encouraged to just read  the italicized  sentences.}Linear, and Multilinear Algebra, Matrix Operations, Decompositions, and Transforms dominate the IoT (Internet of Things), AI (Artificial Intelligence), ML (Machine Learning), and Signal Processing applications. In particular, General Matrix Matrix Multiplication (GEMM) \cite{Thomas21,Thomas22} and the Kronecker Product (KP) 
are the most common \cite{kron1} products. The Khatri-Rao (KR), i.e., parallel KPs, was reported to subsume 90\% of all IoT computation at Siemens in Munich \cite{Acar16}. 
In AI, Recurrent Neural Networks (RNNs) can be difficult to deploy on resource constrained devices.
KPs can compress $\mbox{RNN}$ layers by 16 - 38  times with minimal accuracy loss \cite{Rnn0}. 
Both, MM and KP   occur {\bf often and  in multiples} \cite{Mullin14} within today's software AI tools, e.g., Tensorflow  and Pytorch, written in Python and NumPy. Due to the use of interpretive languages that are utilized to formulate these tools, even with NumPy, and other software accelerators to speed up interpretation, special purpose hardware is being explored, e.g., GPUs and TPUs, as an assist (co-processing).
Even with all this, the necessary speeds and sizes of matrix operations needed are not being realized.

In MoA, the theoretical foundations start with shapes and the Psi indexing function. Together they can define arbitrary array operations that, when composed, yield a semantic/Denotational Normal Form (DNF), or least amount of computation, and memory access, needed for the algorithm while revealing all parallelism. From the DNF, loops bounds are partitioned, "dimension-lifted", to map to the hardware. MoA views the hardware as arrays: indices of data to indices of machine attributes (registers, memories, processors), combined with costs \cite{Mullin88,Gustafson17,Mullin05,conformal}.
MoA 
%is Turing Complete, 
has the Church-Rosser (CR) property \cite{Chetioui19}, and when combined with the Lambda Calculus \cite{Berkling90},  two array programs can be proven equivalent.

%\begin{tcolorbox}[colback=red!5!white,colframe=red!75!black]
%\begin{center}
\vspace{.2cm}
\noindent
{\em Existing array theories and compiler optimizations on array loops, are proper subsets of MoA. All of NumPy's array and tensor operations can be formulated in MoA. In MoA one algorithm, thus, one circuit, describes the Hadamard Product, Matrix Product, Kronecker Product, and Reductions(Contractions) versus four. Consequently less circuitry, power, and energy.}
%\end{center}
%\end{tcolorbox}
\subsection{The Simplicity of MoA: Shapes and the Psi Function}
Although MoA's algebra was influenced by Iverson's APL \cite{Iverson62} and Abram's shapes and indexing tables \cite{Abrams70}, it is MoA's Psi Function, $\psi$, with shapes that defines everything. Any mathematical quality: group, ring, field, ...,  could be added to MoA's indexing calculus. The idea of MoA and Psi Calculus,  starts with a scalar, $\sigma$, and it's shape $\rho \sigma$, an empty vector, denoted by $<>$ or $\Theta$. Since a vector is an array,  it has a  shape, $(\rho <>) \equiv <0>$, the one element vector containing the integer 0, denoting a scalar is a 0-dimensional array. Thus, from the shape, we can determine dimensionality, 
$(\rho (\rho \sigma)) [0] \equiv  <0>[0] \equiv 0$ and the total number of components, $\pi (\rho \sigma)\equiv \pi <> \equiv 1$, in the array. Algorithms on shapes describe how to index arrays with Psi and are defined, such that, Psi takes a valid index vector, or an array
of valid index vectors, and an array as arguments.  For example, in the scalar, $\sigma$, case, $<> \psi \;\sigma$.
% MoA  extends this definition to n-d arrays. 
Next, 2 scalars(0-d) and operations between them can be considered, with an extension to operations with n-dimensional (n-d) arguments. 

\vspace{.2cm}
\noindent
{\em Scalar operations are at the heart of computation, $\sigma_l f \sigma_r$, and in general for n-d arrays, $\xi_l f \xi_r$, where $f$ is an arbitrary scalar function.}

\vspace{.2cm}
Thus, in general, 

\begin{eqnarray}
 \forall\; \vec i \ni 0 \leq^* \vec i <^* \rho \xi_l \nonumber \\
&& \vec i \mbox{ is a valid index vector.}\nonumber \\
 \vec i \psi (\xi_l f \xi_r) & \equiv & (\vec i \psi \xi_l)\; f\; (\vec i \psi \xi_r) \nonumber 
 \end{eqnarray}
 
 \vspace{.2cm}
\noindent
{\em That is, indexing distributes over scalar operations, or in compiler optimization terms, loop fusion.}
% \begin{eqnarray}
 
% \mbox{For a scalar there is only one valid index }, $\vec i$ \mbox{ is } <>, \mbox{ the empty vector}\nonumber \\
\noindent
For a scalar there is only one valid index , $\vec i$  is  $<>$,  the empty vector.
 \[<> \psi  (\sigma_l f \sigma_r)  \equiv  (<> \psi \sigma_l)\; f\;  (<> \psi \sigma_r ) \mbox{(DNF)} \]
 \noindent
 Indexing distributes over scalar operations. \\
 \[\equiv  (\mbox{rav} \;\sigma_l) [\gamma_{row}(<>;<>)] \;f\; (\mbox{rav}\; \sigma_r)[\gamma_{row}(<>;<>)] \]
 \noindent
Relating the DNF to the Operational Normal Form (ONF). 
rav flattens the array in row major.
$\gamma_{row} $ gets the offset using index and shape. \\
\[\equiv  (\mbox{rav} \;\sigma_l)[0] \;f\;(\mbox{rav}\; \sigma_r)[0] 
\mbox{ This is the ONF. }\]
\noindent
Applying the definition of $ \gamma_{row}$  in order to get 0.
\[\equiv (@\sigma_l +0) f (@\sigma_r +0) \mbox{ This is the generic form to build.} \]
%\end{eqnarray}

%\vspace{.2cm}
%\noindent
Bracket Notation relates to the ONF, or how to build the code, through $\gamma$ and pseudo-code, i.e., 
$\mbox{rav} (\vec i \psi \xi) \equiv (\mbox{rav} \;\xi)[\gamma (\vec i; \rho \xi)]$. With a family of gamma, $\gamma$, functions, e.g., row major, column major, a Cartesian index is related to an offset of the array in memory laid out contiguously. {\bf rav} flattens an array based on it's layout. 
Subscripts relate to left or right arguments and superscripts specify dimensionality. Refer to \cite{Mullin88} for all MoA definitions.

\vspace{.2cm}
\noindent
With this, introduce the important identify that is true in general for n-d arrays, denoted by $\xi$:
\[( \iota (\rho \xi)) \psi \xi ) \equiv \xi \] 

{\it This means, with an array's shape, $\rho \xi$, generate an array of indices, $\iota (\rho \xi)$. Then, using that array as an argument to Psi, the original array $\xi$, is returned.}

\vspace{.2cm}
\noindent
In the scalar case, where $\sigma$ denotes a scalar, 
\[ ((\iota (\rho \sigma)) \psi \sigma ) \equiv \sigma \] 
The shape of a scalar is the empty vector $<>$
and, and the only valid index a scalar has is the empty vector, $<>$.
\[ (\iota <>) \psi \sigma \equiv \sigma \]

\[ <> \psi \sigma \equiv \sigma \]
Thus, as long as we can get shapes, e.g., $\rho \xi$, we can get all indices from shapes, e.g., $\iota (\rho \xi))$
that have the properties of the $\psi$ function. This is true in general, no mater what the dimensionality of the array \cite{Mullin88}, including scalars, a 0-dimensional array.

Building upon scalar operations, and extending to scalar vector operations, introduced as {\em scalar extension}, later generalized  as the {\em outer product}. The generalization is completed by adding  {\em reductions/contractions} and, the {\em inner product} (defined using reduction and outer product). Mullin's research connects these four ideas formulated mathematically in MoA; scalar operations: Matrix Multiplication (MM), Hadamard Product (HP), and the Kronecker Product (KP) using {\bf one} algorithm/circuit (ipophp) \cite{Grout18,Grout19}. These designs were extended to {\em Blocked} matrix matrix multiplication by first formulating in MoA, then derived, built, and  tested in C, proving it's performance exceeds modern DGEMM  libraries\cite{Thomas21,Thomas22}. From these experiments, it became clear that a general purpose machine, e.g., cache memory design, languages, Operating Systems (OSes), compilers, ..., would not suffice for optimal array computation. Memory  management, resource management, and the ability to control and optimize array computation was difficult if not impossible.
Much information about the machines was either inaccurate, or was not divulged. Consequently, guided experiments with sophisticated scripts that overlay performance plots, helps  to obtain essential, unknown variables in a developing theoretical MoA model of computation. This information guides the research herein. Research continues to validate that the more shape aware the Operational Normal Form (ONF) is of data and hardware, the easier it is to use special purpose hardware to obtain large amounts/blocks of data(strided DMAs and RMAs, buffers, PIMs,...), that could easily  use  pre-scheduled information of sizes and speeds, up and down the memory hierarchy, {\em deterministically}.

MoA defines all operations using shapes and the Psi indexing function. Hence, when operations are formulated in the MoA algebra, it can be reduced through {\em Psi Reduction} to a semantic/denotational normal form (DNF), i.e., Cartesian indices of all operations are composed.
Then, one of the mapping functions, e.g., $\gamma_{row}$\footnote{There are a whole family of $\gamma$, layout functions: $\gamma_{row},\gamma_{col}, \gamma_{sparse}, etc.$}, transforms an index to an offset in memory, the ONF, or how to build it with knowledge of data layout that capitalizes on starts. stops. and strides \cite{psi-corr}.
Next, formulating dimension lifting, i.e., partitioning shapes, leads to mapping data to hardware \cite{Mullin05}. 
 Combined with Lambda Calculus, iteration, sequence, and control \cite{Berkling90}, we have a Turing complete paradigm to reason about array computation in general.  These fundamentals allow one to define and optimize programs in any domain that use the algebra
 and could be enhanced subsets of 
any language with arrays, e.g., Fortran, Python, or Julia \cite{pythonmoa}. 
 That is, when there is {\bf semantic equivalence} across  programming languages, soft or hard, automatic linear and multi-linear transformations are easily applied, proving correctness by construction. MoA is a {\em Universal Algebra} than can optimize all domain specific languages that use arrays/tensors as their primary data structure.

\subsection{Why MoA Inner and Outer Products?}
Tensor contractions are 3-d extensions of the matrix multiplication \cite{contraction}. Thus, optimizations for higher dimensional
contractions using plus and times (addition and multiplication) are also needed.
In MoA, the formulation of  the inner uses the outer product, noting the  degenerate form of the outer product, is scalar operations. When this is combined with reduction/contraction, i.e., reducing a dimension through addition, or other scalar operation, we have higher dimensional HP, KP, and MMs in one algorithm/circuit (ipophp) or many parallel 2-d versions. An example will help in understanding these concepts.

